Quasi-Perfect State Transfer in Spin Chains via Parametrization of On-Site Energies

In recent years, significant progress has been made in the field of state transfer in spin chains, with the aim of achieving perfect state transfer for quantum information processing applications. Previous research has mainly focused on manipulating inter-site couplings within spin chains; here, we investigate in detail the potential of modifying on-site energies to facilitate precise quantum information transfer. Our findings demonstrate that through targeted adjustments to the diagonal elements of the XY Hamiltonian and leveraging a genetic algorithm, quasi-perfect state transfer can be achieved with careful consideration of the system's spectral characteristics. This investigation into on-site energies offers an alternative approach for achieving high-fidelity state transfer, especially in cases where manipulation of inter-site couplings may be impractical. This study thus represents a significant advancement towards unlocking the diverse applications of spin chains within practical quantum information systems.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements} \label{sec:acknowledgements}
